Towards Hate Speech Detection at Large via Deep Generative Modeling

Hate speech detection is a critical problem in social media platforms, being often accused for enabling the spread of hatred and igniting physical violence. Hate speech detection requires overwhelming resources including high-performance computing for online posts and tweets monitoring as well as thousands of human experts for daily screening of suspected posts or tweets. Recently, Deep Learning (DL)-based solutions have been proposed for automatic detection of hate speech, using modest-sized training datasets of few thousands of hate speech sequences. While these methods perform well on the specific datasets, their ability to detect new hate speech sequences is limited and has not been investigated. Being a data-driven approach, it is well known that DL surpasses other methods whenever a scale-up in train dataset size and diversity is achieved. Therefore, we first present a dataset of 1 million realistic hate and non-hate sequences, produced by a deep generative language model. We further utilize the generated dataset to train a well-studied DL-based hate speech detector, and demonstrate consistent and significant performance improvements across five public hate speech datasets. Therefore, the proposed solution enables high sensitivity detection of a very large variety of hate speech sequences, paving the way to a fully automatic solution.

==> approach-previous.tex <==
\section{The Proposed Approach: Scalable Hate Speech Detection via Data Generation}
%\subsection{Hate Speech Data Generation}
\label{{ssec:approach}}

Ideally, DL-classifiers would be trained on a large and diverse dataset, which 
more truthfully represents the distribution of hate speech, compared with the small datasets that are available as of today (Table~\ref{tab:datasets}). 

in which the examples are drawn independently and identically from the true distribution of the data.

Since the available datsets in Table \ref{tab:datasets} include only few thousands of hate speech examples, their ability to represent the true distribution of hate speech is limited, as evident from the cross-dataset evaluation in Figure \ref{fig:Cross_Dataset}. 

In order to improve the generalization of DL-classifiers we propose a novel approach to augment each dataset in a three-step procedure: (1) Approximating the true distribution of each dataset using the deep generative language model GPT-2 \cite{radford2019language} from OpenAI\footnote{\url{https://openai.com/blog/better-language-models/}}. (2) Sampling from the approximated distribution hundreds of thousands of sequences. (3) Filtering sampled sequences with low probability of being hate speech, by the language representation model BERT \cite{devlin2018bert}. \\
\indent We  divided each dataset to a training set and a testing set using random sampling and a 80\%-20\% split ratio, respectively. The complete workflow as applied to the training set of each source dataset in Table~\ref{tab:datasets} is  summarized in Algorithm~\ref{alg:workflow}.



\begin{comment}
demonstrate the improved generalization capability of a DL classifier, by evaluating the performance using the baseline (un-augmented)  performance of the DL-classifier, to the  using each one of the datasettheir inter- from the  As previously described, the datasets that were used for training hate speech classifiers in previous works are small and has a limited language distribution comparing to real-word scenarios. We seek to enrich these distributions by exposing the classifiers to a much broader language distribution, while staying in the domain of hateful texts.
To do so, we use a pre-trained generative model and its language distribution, and fine-tune it using the datasets described in Table~\ref{tab:datasets}. We then use that fine-tuned model to generated a new, large and diverse hate speech dataset. By using these quality datasets which were carefully collection and annotated we can produce a synthetic dataset at aconsiderably larger scale, hypothesizing to be beneficial for the training and evaluation of a DL-based hate speech classifier
\end{comment}

\begin{algorithm}

%\SetAlgoNoLine
\caption{Dataset Generation}
\small
\label{alg:workflow}
\begin{algorithmic}
    \State {$\mathbf{G}_{hate}$ := GPT-2.fine\_tune($d_{hate}$);}\\
    \State {$ d^{gen}_{hate}$ := $\mathbf{G}_{hate}$.generate();}\\
    \State {BERT.fine\_tune(SST-2);}\\
    \State {BERT.fine\_tune(D);}\\
    \For{$s_{i}\in d^{gen}_{hate}$}
        \State $p_{i} := BERT.predict(s_{i});$
         \IF{$p_{i} == Non-Hate$}
            \State $Remove s_{i} from d^{gen}_{hate};$
         \ELSE
            \State{Continue;}
        \EndIf
    \EndFor 
    \State {$\mathbf{G}_{non-hate}$ := GPT-2.fine\_tune($d_{non-hate}$);}\\
    \State {$ d^{gen}_{non-hate}$ := $\mathbf{G}_{non-hate}$.generate();}\\

    \State {Return $ d^{gen}_{hate}$,   $ d^{gen}_{non-hate}$;}
\end{algorithmic}
\end{algorithm}

\noindent \textbf{Generative  Language Modeling} To generate new data, we used the GPT-2 model \cite{radford2019language}, which is pre-trained on 40GB of the WebText dataset, with an objective of predicting the next word of a sequence given a the previously seen words of that sequence. The GPT-2 model is trained using unsupervised learning to maximize the the likelihood of the sequence's joint probability: \\
\begin{equation}
p(\mathbf{x}) = \coprod_{i=1}^{n} p(s_{i}|s_{1},...,s_{i-1}))    
\end{equation}
\\
where a sequence $\mathbf{x}$ is composed of tokens $(s_{1},\dots\, s_{n})$.
The GPT-2 has been released in four scales:  (i) 117M parameters; (ii) 345M parameters (iii) 764M parameters; and (iv) 1.5B (1542M) parameters, termed GPT-2 XL. Due to computational resources  constraints we chose to use the 764M GPT-2 model, however, as indicated by \cite{radford2019language} choosing the GPT-2 XL leads to significant improvements in NLP tasks, as compared to the 764M model.

\vspace{5 mm}

\noident \textbf{Data Pre-Processing} Tweets typically contain unique elements such as mentions, Re-Tweets, emojis and a multiple punctuation marks (e.g., \emph{\#SlightlyAdjusted RT @CapoToHeaven Alls niggers wanna do is f***, tweet, and drink pineapple soda all day}). To adapt the tweets' style with the GPT-2 requirements we applied the following pre-processing to all input sequences: remove emojis,  RT's, mentions, extra white spaces and repeated characters.

\vspace{5 mm}

\noident \textbf{Distribution Approximation} The process of approximating the probability distribution of a specific class (such as hate or non-hate) is performed by fine-tuning the pre-trained GPT-2 model with the training examples of the required class.  We denote D = $[d_{1},\dots\, d_{n}]$ as the group of source datasets in Table~\ref{tab:datasets}, and $d^{i}_{hate}$, $d^{i}_{non-hate}$ as the samples of $d_{i}$ which belongs to the hate and non-hate classes. we utilized the training set of each source dataset to fine-tune two GPT-2 models: (i) $\mathbf{G}_{hate}$ is fine-tuned over the training samples of $d^{i}_{hate}$ and, (ii) $\mathbf{G}_{non-hate}$ is fine-tuned over the training samples of $d^{i}_{non-hate}$.\\
We denote $ d^{gen}_{hate}}$ as the dataset generated from $\mathbf{G}_{hate}$ fine-tuned over $d^{i}_{hate}$, and a similar notation for the non-hate case as well. By fine-tuning a GPT-2 model for each class of every dataset, the model is exposed to the dataset's unique topics and keywords, and to the specific in-class features.\\


\begin{comment}
Each dataset was randomly divided to a training dataset and a testing dataset using a 80\%-20\% split ratio, respectively. We fine-tuned two GPT-2 models per dataset, one for each class. i.e, for a each dataset we fine-tune a "hate" GPT-2 using only the hate class data, and a "non-hate" GPT-2 fine-tuned by using only the non-hate class data.
\par We denote D = $[d_{1},\dots\, d_{n}]$ as the group of input datasets (see Table~\ref{tab:datasets}), $ d^{gen}_{i}$ as the dataset generated from a GPT-2 fine-tuned with $d_{i}$ and C = $[Hate, Non-Hate]$ as the possible class of each sample (hate$\backslash$non-hate). By fine-tuning a GPT-2 model for each class of every dataset, the model is exposed to the dataset's unique topics and keywords, and to the specific in-class features.\\\vspace{}
\end{comment}
\textbf{Sequences Generation} Using the fine-tuned GPT-2 models, we generated 600K sequences per model. Since the original datasets sequences are relatively short sentences, we generated 30 tokens long sentences with an unconditional setting (i.e., no prompt was given to the GPT-2 model). we used a top\_p parameter of 0.9 and a temperature of 0.9.  See Table \ref{tab:generated_examples} for examples of generated sequences.



\begin{table}[h]
\caption{ROUGE-L scores of data generated  by the GPT-2 language model. All values are close to 0, indicating very low similarity to the source datasets sequences.}
\small
\label{tab:rouge}
\begin{tabular*}{\columnwidth}{ccc}
\toprule
     Source Dataset & Generated Hate & Generated Non-Hate\\\hline\hline
\midrule
{WS} & {0.12} & {0.05}\\
{DV} & {0.07} & {0.052}\\
{FN} & {0.11} & {0.14}\\ 
{WH} & {0.09} & {0.16}\\
{SE} & {0.051} & {0.03}\\
\hline
\hline
\end{tabular*}
\end{table}

\textbf{Sequences Filtering}
While the GPT-2 models that were fine-tuned on the hate class data are expected to generate hateful texts, it is not reasonable to assume that every text generated from these models is indeed hateful. That assumption can not be made because of the very small datasets the GPT-2 is fine-tuned with comparing to its vast pre-trained data (40GB of WikiText). Thus, it is crucial to employ a filter that makes sure, as much as possible, that the generated hate texts are indeed hateful. \par For that reason, we use BERT \cite{devlin2018bert} which is known for its powerful capabilities for many natural language processing tasks. Based on the similarity between the binary case of hate speech detection and the sentiment analysis task, as two binary positive-negative classification tasks, we follow \cite{sun2019fine} who demonstrated the advantages of using BERT as text classifier over several other DL-based classifiers. BERT insert a [CLS] token as the input sequence first position. To utilize BERT as a text classifier, an additional softmax layer is added on top the model's output of the [CLS] token, predicting the class probability. Before fine-tuning the BERT on the hate speech datasets, We empirically found that it is beneficial to further pre-train BERT with the additional softmax layer on similar binary sentiment classification task, Therefore we used the Stanford Sentiment Treebank (SST) described in de Gilbert {\it et al.}~\cite{socher2013recursive, wang2018glue}. We use HuggingFace's platform \cite{Wolf2019HuggingFacesTS} to fine-tune and predict with the BERT model. After BERT computed the logits of each generated sentence, the filtering was performed by taking the generated hate sentences that recieved the highest probability for belonging to the Hate class. The hate speech training of BERT was done on a combined dataset: \begin{enumerate}
    \item combining all hate class sentences of the training sets appearing in Table~\ref{tab:datasets}.
    \item randomly selecting sentences from the combined training sets non-hate class, creating a subset in the same size as the subset described in (1).
\end{enumerate}
\par Finally, BERT scans the generated hate sentences of every fine-tuned GPT-2 model. Sentences which are predicted as non-hate class or hate class with a confidence level below 0.7 filtered out of the generated datasets. 

\vspace{5 mm}

\textbf{Generated Data Diversity}
In order to assess the diversity and originality of the generated data, we utilized the ROUGE-L metric \cite{lin-2004-rouge}, which measures the similarity between computer-generated text  and human-written text. ROUGE-L is a \emph{Longest Common Subsequence} (LCS) based measure that indicates how much is in common between two word sequences, ranging from 0 (nothing) to 1 (identical sequences). Table~\ref{tab:rouge} shows the average score for each of the original datasets and their corresponding generated datasets.  All values are close to zero, clearly indicating very low similarity between the generated sequences and the ones in the source datasets that were used to fine-tune the GPT-2 model. These results confirm the high-level of originality of the generated hate and non-hate sequences.



==> biography.tex <==
\begin{comment}

\begin{IEEEbiography}{First A. Author}{\,}current employment (is
currently with XYZ Corporation, New York, NY, USA). Author's latest degree received or which he/she is currently pursuing (He received the B.S. degree and the M.S. degree...."). Author's research interest. Association with any official journals or conferences; major professional and/or academic achievements, i.e., best paper awards, research grants, etc.; any publication information (number of papers and titles of books published). Author membership information, e.g., is a member of the IEEE and the IEEE Computer Society, if applicable, is noted at the end of the biography. Biography is limited to single paragraph only (He is a member of IEEE, etc.). All biographies should be limited to one paragraph, five to six sentences, consisting of the following: (e.g., ``Dr. Author received a B.S. degree and an M.S. degree $\ldots$.''), including years achieved; association with any official journals or conferences; major professional and/or academic achievements, i.e., best paper awards, research grants, etc.; any publication information (number of papers and titles of books published); current research interests; association with any professional associations. Author membership information, e.g., is a member of the IEEE and the IEEE Computer Society, if applicable, is noted at the end of the biography. Contact him/her at faauthor@xyz.com.
\end{IEEEbiography}

\begin{IEEEbiography}{Amir Adler}{\,}is a Senior Lecturer at the Electrical Engineering Department, Braude College of Engineering, Israel, and a Research Affiliate at the McGovern Institute for Brain Research, MIT. Previously, he was a post-doctoral associate at the Center for Brains, Minds, and Machines (CBMM), MIT, where his research was focused on deep learning. He served as the Chief Scientist of the Ministry of Communications, Israel, and was Chief Technology Officer of the Wi-Fi division at NextWave Wireless Inc. (acquired by AT\&T). He is the recipient of the 2011 Google Europe Doctoral Fellowship in Multimedia, a co-recipient of the 2012 HP Labs Open Innovation Research Award, and a recipient of the 2019 Facebook Research Content Policy Research award. His current research interests are deep learning and brain source localization. Dr. Adler received a B.Sc (Cum Laude) in Electrical Engineering, an M.Eng (Cum Laude) in Electrical Engineering, and a PhD in Computer Science, all from the Technion - Israel Institute of Technology. \\
\end{IEEEbiography}

\begin{IEEEbiography}{Third C. Author, III,}{\,}is with DEF Corporation, Tokyo, Japan. Dr. Author's biography appears here.  Contact him/her at tcauthor@def.com.
\end{IEEEbiography}
\end{comment}

==> cross.tex <==
\begin{table*}[h]
\caption{Cross-Dataset performance evaluation with the augmented training sets.}
\large
\label{tab:cross_dataset}
\resizebox{\textwidth}{!}{
\begin{tabular}{cc|ccc|ccc|ccc|ccc}

\toprule
     Source & Target &  \multicolumn{3}{c}{Accuracy} & \multicolumn{3}{c}{Precision} & \multicolumn{3}{c}{Recall} & \multicolumn{3}{c}{F1} \\ 

     Dataset & Dataset \midrule& Baseline & Augmented & (\%) & Baseline & Augmented & (\%) & Baseline & Augmented & (\%) & Baseline & Augmented &(\%)\\\hline
{DV} & {WH} & {0.794} & {0.82} & {+3.27} & {0.278} & {0.441} & {58.63} & {0.189} & {0.507} & {+168.25} & {0.225} & {0.472} & {+109.77}\\
{DV} & {WS} & {0.652} & {0.832} & {+27.6} & {0.471} & {0.87} & {+84.71} & {0.107} & {0.599} & {+459.81} & {0.174} & {0.709} & {+307.47}\\
{FN} & {SE} & {0.613} & {0.645} & {+5.22} & {0.689} & {0.57} & {-17.27} & {0.155} & {0.644} & {+315.48} & {0.253} & {0.605} & {+139.13}\\
{FN} & {WH} & {0.846} & {0.85} & {0.472} & {0.636} & {0.528} & {-16.98} & {0.063} & {0.507} & {+704.76} & {0.114} & {0.517} & {+353.5}\\
{WH} & {DV} & {0.752} & {0.777} & {+3.32} & {0.714} & {0.61} & {-14.56} & {0.053} & {0.364} & {+586.79} & {0.099} & {0.456} & {+360.6}\\
{WH} & {SE} & {0.584} & {0.593} & {+1.54} & {0.572} & {0.522} & {-8.74} & {0.069} & {0.45} & {+552.17} & {0.124} & {0.484} & {+290.32}\\
{SE} & {FN} & {0.926} & {0.924} & {-0.216} & {0.694} & {0.489} & {-29.53} & {0.031} & {0.226} & {+629.03} & {0.059} & {0.309} & {+423.72}\\
{SE} & {WS} & {0.662} & {0.754} & {+13.89} & {0.875} & {0.872} & {-0.34} & {0.017} & {0.331} & {+1,847.06} & {0.034} & {0.48} & {+1,311.76}\\
{WS} & {WH} & {0.749} & {0.824} & {+10.01} & {0.332} & {0.45} & {+35.54} & {0.579} & {0.489} & {-15.54} & {0.422} & {0.469} & {+11.13}\\
{WS} & {FN} & {0.822} & {0.895} & {+8.88} & {0.135} & {0.233} & {+72.59} & {0.255} & {0.176} & {-30.98} & {0.177} & {0.201} & {+13.55}\\
\bottomrule
\end{tabular}
}
\end{table*}

==> temp.tex <==
from the social media platforms. have long been a prominent topic in social media research, a large share of research done in recent years is based on small datasets which are non-representative of a true language distribution.
Ideally, a Deep Learning based Hate speech classifier should be exposed to a large and diverse dataset, with implicit and explicit hateful meanings, in order to be able to distinguish between hate and non-hate texts in the scale and complexity of real-world scenarios.
Training a classifier on such datasets may lead to a large generalization error.
Creating a large, annotated hate speech dataset that could potentially reduce a classifier's generalization error can be a long and expensive process.
In this work we tackle these challenges by being the first to enrich an existing hate speech dataset using a deep generative model, creating a very large synthetic hate speech datasets and employing them for training a hate speech classifier. We demonstrate the how the synthetic dataset can assist with reducing the generalization error, and also exhibit the quality of the synthetic data and its diversification.

\begin{comment}
\par Therefore, it is crucial to have a diverse and quality dataset when conducting a hate speech detection research.
Many of the publicly available datasets are collected using the Twitter API and are bound to its policies. Thus, only the tweet IDs are available yet their content needs to be retrieved. that could cause a problem when the tweet itself is removed for any reason, causing the dataset to shrink dramatically.
In addition, since tweets are generally made of very few number of words, performing some types of pre-processing \cite{zhang2018detecting} might reduce it to even shorter and potentially less informative word sequences.


\begin{table*}
\caption{The generalization error is shown in almost every parameter. The classifier was trained on the training set of DV dataset and evaluated on a held-out sets of DV and WS. Both datasets are tweets collected from Twitter and labeled as hate or non-hate.}\label{tab:generalization_err}
\centering
\begin{tabular}{cccccc}
\hline
Training Dataset & Evaluation Dataset & Accuracy & Precision & Recall & F1 \\
\hline
DV & DV & 91.4 & 93.4 & 71.7 & 81.2\\
DV & FN & 92.8 & 52.5 & 40 & 45.4\\
\hline
Change & & 1.53 & \textbf{-43.8\%} & \textbf{-44.2\%} & \textbf{-44.08\%}\\
\end{tabular}
\end{table*}
\label{tab:generalization_err}
\end{comment}

The evaluation is considering both standard classification performance measurements, as well as the improvement over the classifier's generalization error. The experiments setup include a baseline and an augmented configuration.

\indent We trained and evaluated a classifier with the architecture described in \cite{zhang2018detecting} using each of the datasets described in Table~\ref{tab:datasets}.
\ident We considered three settings: 
\begin{enumerate}
    \item \textbf{Baseline} - Train and evaluate the classifier on each dataset by applying a 80-20 train-test split. A combined datasets setting was also evaluated, where all the datasets were merged into a single dataset and a 80-20 split was applied.
    \item \textbf{Augmentation} - Repeat the same experiment described above, with the difference of augmenting the training set using synthetic sentences that were generated from two GPT-2 models that were fine-tuned on the dataset that is being evaluated (one model for each class).
    \item \textbf{Cross-Dataset} - Perform a Baseline and an Augmentation experiment, by training the classifier on a certain dataset (and augmenting the data with a GPT-2 model fine-tuned on that dataset) and evaluate the classifier on a held-out set which belongs to a different dataset.
\end{enumerate}

This process, although guaranteeing high quality ground truth data, is long, expensive and may suffer from inherent biases, like amateur annotators or misleading labeling instructions. The collection process also struggles with collecting a \textbf{representative dataset}, since it is limited to the language distribution of a small dataset which can not grasp all possible forms of hate speech and possible terms. Thus, having a modest-sized, high-quality dataset does not guarantee that a classifier trained with such dataset will be able to handle such complexities.

\begin{comment}
 \begin{figure*}[h]
  \centering
  \begin{minipage}[b]{0.485\textwidth}
    \includegraphics[scale=0.59]{semeval.jpg}
    \floatfoot{\small (a) SE dataset.}
  \end{minipage}
  \begin{minipage}[b]{0.485\textwidth}
   \includegraphics[scale=0.59]{founta.jpg}
    \floatfoot{\small (b) FN dataset.}
  \end{minipage}\\
  \vskip 10pt
  \centering
  \begin{minipage}[b]{0.485\textwidth}
   \includegraphics[scale=0.59]{davidson.jpg}
    \floatfoot{\small (c) DV dataset.}
  \end{minipage}
  \begin{minipage}[b]{0.485\textwidth}
   \includegraphics[scale=0.59]{white.jpg}
   \floatfoot{\small (d) WH dataset.}
  \end{minipage}\\
    \vskip 10pt
    \centering
      \begin{minipage}[b]{0.485\textwidth}
   \includegraphics[scale=0.59]{waseem.jpg}
   \floatfoot{\small (e) WS dataset.}
  \end{minipage}
  \begin{minipage}[b]{0.485\textwidth}
   \includegraphics[scale=0.59]{combined.jpg}
   \floatfoot{\small (f) Combined dataset.}
  \end{minipage}
  \caption{Precision-Recall curves of the Hate Speech detector, trained separately using each dataset (a)-(e) and using the combined dataset (f), comparing baseline and augmented train data results. }
  \label{fig:PR-Curves}
\end{figure*}
\end{comment}     


\begin{comment}
\begin{figure*}
\label{fig:cross_charts}

 \begin{minipage}{0.45\textwidth}
 \centering
 \includegraphics[trim={0.25cm 3.5cm 0cm 3.5cm},clip ,width=37.5pc]{cross_chart_a.png}
 \end{minipage}\\
 \begin{minipage}{0.45\textwidth}
 \centering
 \includegraphics[trim={0.25cm 3.5cm 0cm 4.5cm},clip ,width=37.5pc]{cross_chart_b.png}
 \end{minipage}
 \caption{Cross-Dataset experiment results. The Baseline bar (blue) shows the result of each metric when both training and test sets are from the same dataset (left side of each pair.) The Cross-Dataset bar (red) demonstrates the cross setting, where the detector is trained on a training set from one dataset (left) and evaluated on a test set from another (right). Cross with Augmentation refers to the same setting as the Cross-Dataset, with the addition of generated data augmenting the training set.  }
\end{figure*}
\end{comment}
%\begin{appendices}
%\section{Precision-Recall Curves}
\begin{comment}

 \begin{figure*}[h]
  \centering
  \begin{minipage}[b]{0.45\textwidth}
    \includegraphics[scale=0.56]{semeval.jpg}
    \floatfoot{\small SE Precision-Recall curve.}
  \end{minipage}
  \begin{minipage}[b]{0.45\textwidth}
   \includegraphics[scale=0.56]{founta.jpg}
    \floatfoot{\small FN Precision-Recall curve.}
  \end{minipage}

\end{figure*}

 \begin{figure*}[h]
  \centering
  \begin{minipage}[b]{0.45\textwidth}
   \includegraphics[scale=0.56]{davidson.jpg}
    \floatfoot{\small DV Precision-Recall curve.}
  \end{minipage}
  \begin{minipage}[b]{0.45\textwidth}
   \includegraphics[scale=0.56]{white.jpg}
   \floatfoot{\small WH Precision-Recall curve.}
  \end{minipage}
\end{figure*}

\begin{figure*}[h]
    \centering
      \begin{minipage}[b]{0.45\textwidth}
   \includegraphics[scale=0.56]{waseem.jpg}
   \floatfoot{\small WS Precision-Recall curve.}
  \end{minipage}
  \begin{minipage}[b]{0.45\textwidth}
   \includegraphics[scale=0.56]{combined.jpg}
   \floatfoot{\small Combined datasets Precision-Recall curve.}
  \end{minipage}
\end{figure*}
\end{comment}

\begin{comment}
\begin{table*}[h]
\caption{Cross-Dataset performance, comparing detector training with  baseline to augmented-baseline training sets.}

\label{tab:cross_dataset}
\resizebox{\textwidth}{!}{
\large
\begin{tabular}{cc|ccc|ccc|ccc|ccc}

\toprule
     Source & Target  &  \multicolumn{3}{c}{Accuracy} & \multicolumn{3}{c}{Precision} & \multicolumn{3}{c}{Recall} & \multicolumn{3}{c}{F1} \\ 

     Dataset & Dataset  \midrule& Baseline & Augmented & (\%) & Baseline & Augmented & (\%) & Baseline & Augmented & (\%) & Baseline & Augmented &(\%)\\\hline
{FN} & {SE} & {0.613} & {0.645} & {+5.22} & {0.689} & {0.57} & {-17.27} & {0.155} & {0.644} & {+315.48} & {0.253} & {0.605} & {+139.13}\\
{FN} & {WH} & {0.846} & {0.85} & {0.472} & {0.636} & {0.528} & {-16.98} & {0.063} & {0.507} & {+704.76} & {0.114} & {0.517} & {+353.5}\\
{DV} & {WH} & {0.794} & {0.82} & {+3.27} & {0.278} & {0.441} & {+58.63} & {0.189} & {0.507} & {+168.25} & {0.225} & {0.472} & {+109.77}\\
{DV} & {WS} & {0.652} & {0.832} & {+27.6} & {0.471} & {0.87} & {+84.71} & {0.107} & {0.599} & {+459.81} & {0.174} & {0.709} & {+307.47}\\
{SE} & {WS} & {0.662} & {0.754} & {+13.89} & {0.875} & {0.872} & {-0.34} & {0.017} & {0.331} & {+1,847.06} & {0.034} & {0.48} & {+1,311.76}\\
{SE} & {FN} & {0.926} & {0.924} & {-0.216} & {0.694} & {0.489} & {-29.53} & {0.031} & {0.226} & {+629.03} & {0.059} & {0.309} & {+423.72}\\
{WH} & {SE} & {0.584} & {0.593} & {+1.54} & {0.572} & {0.522} & {-8.74} & {0.069} & {0.45} & {+552.17} & {0.124} & {0.484} & {+290.32}\\
{WH} & {DV} & {0.752} & {0.777} & {+3.32} & {0.714} & {0.61} & {-14.56} & {0.053} & {0.364} & {+586.79} & {0.099} & {0.456} & {+360.6}\\
{WS} & {WH} & {0.749} & {0.824} & {+10.01} & {0.332} & {0.45} & {+35.54} & {0.579} & {0.489} & {-15.54} & {0.422} & {0.469} & {+11.13}\\
{WS} & {FN} & {0.822} & {0.895} & {+8.88} & {0.135} & {0.233} & {+72.59} & {0.255} & {0.176} & {-30.98} & {0.177} & {0.201} & {+13.55}\\
\bottomrule
\end{tabular}
}
\end{table*}
\end{comment}

\subsection{Cross Dataset Performance}
\label{ssec:generalization}
As will be further described below, previous works tended to train and evaluate a classifier on a small and imbalanced dataset. \par We claim that this type of framework may lead to a large generalization error, that will prevent the classifier from identifying a large portion of hateful texts. \par To get a first look at this problem, we show an experiment where a hate speech classifier is trained and evaluated on a certain dataset (with hate$\backslash$non-hate classes) and evaluated again on a different dataset that has the same properties. Figure ~\ref{fig:Cross_Dataset} clearly shows the decrease in the classifier's performance.


indent Performance was evaluated using standard classification metrics: Accuracy (A), Precision (P) - The proportion of samples predicted as positive by the detector that are truly positive,
Recall (R) - termed also \textit{Sensitivity}, is the proportion of all positive samples that were correctly identified as positive by the detector, and F1 - the harmonic mean of precision and recall. The formal definition of each metric is given in the following:\\

$A =\frac{Total Correct}{Total Samples}=\frac{TP+TN}{TP+FP+TN+FN}$\\

$P =\frac{True Positive}{Total Selected Positive}=\frac{TP}{TP+FP}$\\

$R=\frac{True Positive}{Total Actual Positive}=\frac{TP}{TP+FN}$\\

$F_{1}=2 \frac{P \times R}{P + R}$
